Spams meet Cryptocurrencies: Sextortion in the Bitcoin Ecosystem

In the past year, a new spamming scheme has emerged: sexual extortion messages requiring payments in the cryptocurrency Bitcoin, also known as sextortion. This scheme represents a first integration of the use of cryptocurrencies by members of the spamming industry. Using a dataset of 4,340,736 sextortion spams, this research aims at understanding such new amalgamation by uncovering spammers' operations. To do so, a simple, yet effective method for projecting Bitcoin addresses mentioned in sextortion spams onto transaction graph abstractions is computed over the entire Bitcoin blockchain. This allows us to track and investigate monetary flows between involved actors and gain insights into the financial structure of sextortion campaigns. We find that sextortion spammers are somewhat sophisticated, following pricing strategies and benefiting from cost reductions as their operations cut the upper-tail of the spamming supply chain. We discover that one single entity is likely controlling the financial backbone of the majority of the sextortion campaigns and that the 11-month operation studied yielded a lower-bound revenue between \$1,300,620 and \$1,352,266. We conclude that sextortion spamming is a lucrative business and spammers will likely continue to send bulk emails that try to extort money through cryptocurrencies.

==> tables/active_clusters.tex <==
\begin{tabular}{rrrrr}
\toprule
{} &    Cluster & \#Seed Addresses & \#Addresses &             Spent &             First Tx \\
\midrule
41 &  296152187 &               1 &    398,777 &  2,155,478,410.82 &  2013-03-22 20:00:00 \\
50 &  363386240 &               3 &    564,595 &  2,110,090,569.45 &  2016-03-21 16:10:22 \\
29 &  436416240 &              16 &         52 &        240,220.82 &  2018-09-25 17:50:12 \\
10 &  472568332 &              15 &         25 &        200,146.04 &  2019-01-07 13:21:09 \\
11 &  461061700 &              13 &         22 &        178,244.54 &  2018-10-30 21:50:39 \\
2  &  456990025 &               6 &         19 &        108,651.51 &  2018-10-25 10:19:19 \\
34 &  440183283 &              13 &         37 &        103,660.49 &  2018-09-12 11:53:20 \\
1  &  431970097 &               8 &         29 &         77,061.92 &  2018-09-10 07:53:14 \\
40 &  479316543 &               3 &         11 &         50,105.61 &  2019-01-24 13:21:59 \\
16 &  443041123 &              11 &         47 &         36,660.63 &  2018-10-15 19:34:26 \\
\bottomrule
\end{tabular}


==> tables/basket_seeds_clusters_expanded.tex <==
\begin{tabular}{rrrr}
\toprule
Basket & \#Seed Addresses & \#Clusters & \#Expanded Addresses \\
\midrule
     0 &               2 &         2 &                  23 \\
     1 &               4 &         3 &                  85 \\
     2 &              46 &        44 &             398,816 \\
     3 &              17 &         9 &                  52 \\
     4 &              21 &        19 &                  27 \\
     5 &               1 &         1 &                  28 \\
     6 &               1 &         1 &                  36 \\
     7 &               2 &         2 &                  34 \\
     8 &              30 &        23 &                   0 \\
     9 &               8 &         4 &                  33 \\
    10 &               2 &         2 &                  25 \\
    11 &               4 &         3 &                  62 \\
    12 &              22 &        21 &                  68 \\
    13 &               3 &         3 &                  24 \\
    14 &          10,460 &    10,459 &                   0 \\
    16 &               1 &         1 &                  24 \\
    17 &             991 &       954 &                   0 \\
    18 &               2 &         2 &                  23 \\
    19 &               1 &         1 &                  18 \\
    20 &              14 &         7 &                 126 \\
    21 &               1 &         1 &                  36 \\
    22 &               2 &         2 &                  64 \\
    24 &               5 &         4 &                   1 \\
    25 &             535 &       535 &                   0 \\
    26 &              12 &        12 &                  44 \\
    28 &               1 &         1 &                  24 \\
    30 &              14 &         9 &                  71 \\
    31 &               2 &         2 &                   3 \\
    32 &              11 &        11 &                 107 \\
    41 &              56 &        46 &                   0 \\
    44 &               6 &         1 &                  41 \\
    45 &               1 &         1 &                  28 \\
    47 &              12 &        11 &                  59 \\
    53 &               3 &         3 &                   1 \\
    59 &              65 &        65 &                   0 \\
    64 &               1 &         1 &                  10 \\
    66 &              42 &        42 &                   0 \\
    71 &               1 &         1 &                   8 \\
    73 &               3 &         1 &             564,592 \\
    75 &              36 &        36 &                   0 \\
    76 &               3 &         2 &                  63 \\
    77 &               1 &         1 &                  18 \\
    80 &               3 &         1 &                   1 \\
    85 &               3 &         2 &                  63 \\
    91 &               1 &         1 &                  51 \\
    95 &              18 &        18 &                   0 \\
    97 &               1 &         1 &                  21 \\
   100 &              16 &        15 &                   0 \\
   101 &               3 &         1 &                  34 \\
   111 &               1 &         1 &             564,594 \\
   112 &              12 &        12 &                   0 \\
   115 &              10 &        10 &                   0 \\
   120 &               1 &         1 &                  36 \\
   121 &               8 &         8 &                   0 \\
   122 &               1 &         1 &                   0 \\
   124 &               1 &         1 &                   0 \\
   127 &               8 &         8 &                   0 \\
   133 &               1 &         1 &                  51 \\
   139 &               7 &         7 &                   0 \\
   142 &               6 &         5 &                  41 \\
   154 &               6 &         6 &                   0 \\
   174 &               1 &         1 &                   0 \\
   187 &               4 &         4 &                   0 \\
   198 &               3 &         3 &                   0 \\
   201 &               3 &         3 &                   0 \\
   205 &               2 &         2 &                   2 \\
   212 &               1 &         1 &                   0 \\
   216 &               1 &         1 &                   0 \\
   220 &               1 &         1 &                   0 \\
   225 &               1 &         1 &                   0 \\
   232 &               3 &         3 &                   5 \\
   247 &               2 &         2 &                   0 \\
   253 &               1 &         1 &                   7 \\
   276 &               2 &         2 &                   6 \\
   277 &               1 &         1 &                   0 \\
   293 &               2 &         2 &                  54 \\
   298 &               1 &         1 &                   2 \\
   388 &               1 &         1 &                  24 \\
   416 &               1 &         1 &                   5 \\
   485 &               1 &         1 &                   3 \\
   518 &               1 &         1 &                   0 \\
   531 &               1 &         1 &                   0 \\
   717 &               1 &         1 &                   0 \\
 1,084 &               1 &         1 &                   0 \\
 1,376 &               1 &         1 &                   0 \\
 1,378 &               1 &         1 &                   0 \\
 1,420 &               1 &         1 &                   2 \\
 1,619 &               1 &         1 &                   3 \\
 1,644 &               1 &         1 &                  29 \\
 1,748 &               1 &         1 &                   5 \\
 1,799 &               1 &         1 &                   2 \\
\bottomrule
\end{tabular}


==> tables/baskets_table.tex <==
\begin{tabular}{rllrlllrr}
\toprule
Basket & Campaign & Language &    \#Emails &      Range [\$] & Currency &            Time Period & \#Passwords (Unique) & Jaccard Mean (Var) \\
\midrule
     0 &        A &       cs &  1,811,062 &      280 | 290 &      EUR &  2018-12-02|2018-12-23 &   387,943 (283,828) &         0.98 (0.0) \\
     1 &        E &       cs &    594,904 &      250 | 550 &      USD &  2018-09-06|2018-11-12 &   544,448 (388,809) &         0.96 (0.0) \\
     2 &        B &       en &    415,925 &    300 | 7,000 &      USD &  2018-09-22|2019-01-24 &   414,785 (297,514) &         0.91 (0.0) \\
     3 &        C &       en &    345,969 &      695 | 899 &      USD &  2018-10-29|2019-02-12 &   303,910 (234,354) &         0.92 (0.0) \\
     4 &        A &       en &    331,742 &    500 | 1,000 &  USD,EUR &  2018-11-30|2019-02-13 &               0 (0) &        0.82 (0.01) \\
     5 &        G &       cs &    256,252 &      200 | 290 &      USD &  2018-09-27|2018-11-06 &   256,252 (189,173) &         0.98 (0.0) \\
     6 &        D &       cs &    186,723 &      250 | 250 &      USD &  2018-09-03|2018-11-24 &               0 (0) &          1.0 (0.0) \\
     7 &        F &       en &    146,709 &      700 | 750 &      USD &  2018-12-20|2019-02-15 &    111,114 (97,485) &         0.94 (0.0) \\
     8 &        L &       en &    100,395 &      700 | 999 &      USD &  2018-10-14|2019-01-15 &     54,883 (49,721) &        0.86 (0.01) \\
     9 &        C &       en &     44,790 &    500 | 1,000 &      USD &  2018-09-09|2018-12-27 &     44,454 (26,920) &         0.93 (0.0) \\
    10 &        A &       de &     19,850 &      336 | 784 &      EUR &  2018-12-07|2019-01-21 &               0 (0) &         0.99 (0.0) \\
    11 &        E &       ko &     19,683 &      400 | 500 &      USD &  2018-09-14|2018-12-26 &               0 (0) &          1.0 (0.0) \\
    12 &        G &       en &     18,314 &    200 | 2,000 &      USD &  2018-09-18|2019-02-13 &               0 (0) &        0.79 (0.03) \\
    13 &        C &       de &     13,732 &      336 | 504 &      EUR &  2018-11-24|2019-01-22 &               0 (0) &         0.99 (0.0) \\
    14 &        F &       en &     12,476 &    500 | 7,000 &      USD &  2018-09-13|2019-01-15 &      12,213 (1,472) &         0.45 (0.0) \\
    16 &        A &       pl &      5,128 &      285 | 285 &      EUR &  2019-01-15|2019-01-20 &               0 (0) &          1.0 (0.0) \\
    17 &        I &       en &      5,059 &      900 | 900 &      USD &  2018-10-29|2018-11-28 &         5,058 (584) &         0.49 (0.0) \\
    18 &        A &       it &      2,196 &      224 | 896 &      EUR &  2018-12-25|2019-01-19 &               0 (0) &         0.99 (0.0) \\
    19 &        D &       de &      2,124 &      500 | 599 &      USD &  2018-09-29|2018-10-27 &               0 (0) &         0.56 (0.0) \\
    20 &        C &       en &      1,061 &      615 | 899 &      USD &  2018-10-27|2019-02-06 &         1,060 (429) &        0.88 (0.01) \\
    21 &        E &       pl &        955 &      300 | 300 &      USD &  2018-09-14|2018-10-13 &               0 (0) &         0.99 (0.0) \\
    22 &        E &       de &        901 &      300 | 350 &      USD &  2018-09-13|2018-10-11 &               0 (0) &         0.99 (0.0) \\
    24 &        T &       en &        823 &      560 | 560 &      EUR &  2019-01-09|2019-01-10 &               0 (0) &         0.99 (0.0) \\
    25 &        I &       en &        762 &      900 | 900 &      USD &  2018-10-27|2018-10-28 &           761 (753) &         0.49 (0.0) \\
    26 &        N &       en &        683 &    300 | 2,240 &  USD,EUR &  2018-10-21|2019-01-14 &           370 (367) &         0.54 (0.0) \\
    28 &        A &       es &        616 &      200 | 299 &      USD &  2019-01-01|2019-01-22 &               0 (0) &         0.99 (0.0) \\
    30 &        D &       en &        523 &      200 | 800 &      USD &  2018-09-25|2019-02-13 &           514 (195) &        0.87 (0.01) \\
    31 &        P &       en &        502 &  1,000 | 1,000 &      USD &  2018-09-25|2019-02-13 &             43 (28) &         0.97 (0.0) \\
    32 &        E &       en &        499 &      200 | 800 &      USD &  2018-09-15|2019-02-13 &           436 (121) &        0.87 (0.01) \\
    41 &        B &       en &        355 &    200 | 1,000 &      USD &  2018-11-06|2019-02-13 &               0 (0) &        0.96 (0.02) \\
    44 &        S &       en &        311 &      500 | 625 &      USD &  2018-10-22|2018-10-28 &           202 (199) &         0.53 (0.0) \\
    45 &        G &       it &        271 &      300 | 300 &      USD &  2018-10-15|2018-10-17 &               0 (0) &         0.99 (0.0) \\
    47 &        I &       en &        263 &      500 | 900 &      USD &  2018-10-22|2019-02-07 &           251 (138) &        0.59 (0.07) \\
    53 &        Q &       en &        130 &      801 | 899 &      USD &  2018-10-29|2018-11-09 &           130 (130) &        0.46 (0.01) \\
    59 &        U &       en &         66 &  1,000 | 1,000 &      USD &  2019-01-21|2019-01-22 &               0 (0) &         0.69 (0.0) \\
    64 &        A &       nl &         58 &      392 | 402 &      EUR &  2019-02-06|2019-02-07 &               0 (0) &        0.91 (0.01) \\
    66 &        V &       en &         50 &    800 | 5,000 &      USD &                    0|0 &               0 (0) &         0.43 (0.0) \\
    71 &        C &       fr &         44 &      338 | 443 &      EUR &  2019-02-11|2019-02-13 &               0 (0) &         0.99 (0.0) \\
    73 &        W &       en &         40 &    950 | 1,270 &  GBP,USD &  2018-10-24|2019-01-09 &               0 (0) &        0.72 (0.04) \\
    75 &        F &       en &         36 &    300 | 7,000 &      USD &  2018-09-16|2019-02-13 &             18 (14) &        0.39 (0.01) \\
    76 &        B &       es &         36 &      200 | 250 &      USD &  2018-09-21|2018-10-15 &               0 (0) &         0.98 (0.0) \\
    77 &        D &       de &         35 &      501 | 599 &      USD &  2018-10-25|2018-10-27 &               0 (0) &        0.66 (0.01) \\
    80 &        J &       sk &         30 &      450 | 450 &      USD &  2018-09-30|2018-10-15 &               0 (0) &        0.88 (0.01) \\
    85 &        B &       sv &         27 &      700 | 700 &      USD &  2018-09-23|2018-09-29 &               0 (0) &         0.99 (0.0) \\
    91 &        B &       it &         23 &      450 | 450 &      USD &  2018-09-24|2018-09-26 &               0 (0) &         0.99 (0.0) \\
    95 &        X &       en &         20 &      200 | 500 &      USD &  2019-02-10|2019-02-13 &               0 (0) &         0.71 (0.0) \\
    97 &        C &       it &         19 &      280 | 290 &      EUR &  2018-12-05|2018-12-07 &               0 (0) &         0.99 (0.0) \\
   100 &        L &       en &         17 &    927 | 7,000 &      USD &  2018-09-18|2018-12-11 &               0 (0) &        0.42 (0.05) \\
   101 &        D &       sv &         17 &      600 | 700 &      USD &  2018-09-21|2018-10-10 &               0 (0) &         0.97 (0.0) \\
   111 &        O &       en &         12 &      880 | 980 &      USD &                    0|0 &               0 (0) &        0.84 (0.01) \\
   112 &        F &       en &         12 &    976 | 6,000 &      USD &  2018-09-15|2018-12-10 &             12 (11) &        0.41 (0.02) \\
   115 &        F &       en &         11 &  1,000 | 7,000 &      USD &  2018-09-13|2018-10-05 &             10 (10) &         0.41 (0.0) \\
   120 &        D &       it &         10 &      300 | 300 &      USD &  2018-09-25|2018-09-26 &               0 (0) &         0.99 (0.0) \\
   121 &        K &       en &         10 &      380 | 930 &  USD,EUR &  2018-10-01|2018-12-13 &               0 (0) &         0.38 (0.0) \\
   122 &        C &       en &         10 &  1,000 | 1,000 &      USD &  2018-12-03|2018-12-03 &               0 (0) &         0.99 (0.0) \\
   124 &        Y &       en &         10 &      822 | 897 &      USD &  2018-10-28|2018-10-29 &               0 (0) &         0.41 (0.0) \\
   127 &        Z &       en &          9 &  1,200 | 3,000 &      USD &  2018-09-14|2018-09-20 &               0 (0) &         0.37 (0.0) \\
   133 &        B &       ko &          9 &      500 | 500 &      USD &  2018-09-24|2018-09-25 &               0 (0) &         0.99 (0.0) \\
   139 &       AA &       en &          8 &      200 | 500 &      USD &  2019-02-11|2019-02-13 &               8 (7) &         0.89 (0.0) \\
   142 &        B &       en &          8 &    800 | 5,000 &      USD &  2018-09-17|2018-10-16 &               8 (8) &        0.59 (0.04) \\
   154 &       BB &       en &          6 &      450 | 880 &      USD &  2018-09-22|2018-09-24 &               0 (0) &         0.49 (0.0) \\
   174 &        A &       no &          5 &      550 | 550 &      NOK &  2018-12-16|2018-12-17 &               0 (0) &          1.0 (0.0) \\
   187 &        K &       en &          4 &      550 | 890 &      USD &  2018-09-16|2018-09-18 &               0 (0) &         0.37 (0.0) \\
   198 &       CC &       en &          3 &      610 | 840 &      USD &  2018-09-25|2018-10-12 &               0 (0) &         0.56 (0.0) \\
   201 &        F &       en &          3 &  2,000 | 2,000 &      USD &  2018-09-22|2018-10-18 &               3 (3) &         0.47 (0.0) \\
   205 &        J &       it &          3 &      300 | 300 &      USD &  2018-09-21|2018-09-25 &               0 (0) &         0.98 (0.0) \\
   212 &       DD &       en &          3 &      710 | 710 &      USD &  2018-12-11|2018-12-11 &               0 (0) &          1.0 (0.0) \\
   216 &        O &       en &          3 &      980 | 980 &      USD &                    0|0 &               0 (0) &         0.89 (0.0) \\
   220 &       EE &       sk &          3 &          0 | 0 &      BTC &  2018-11-08|2018-11-08 &               0 (0) &          1.0 (0.0) \\
   225 &       FF &       en &          3 &      358 | 470 &      EUR &  2019-01-08|2019-01-08 &               0 (0) &         0.37 (0.0) \\
   232 &        H &       en &          3 &      336 | 448 &      EUR &  2018-09-15|2018-09-15 &               0 (0) &          0.4 (0.0) \\
   247 &        J &       it &          2 &      490 | 500 &      USD &  2018-11-03|2018-11-05 &               0 (0) &          0.9 (0.0) \\
   253 &        H &       en &          2 &      336 | 672 &      EUR &  2018-09-14|2018-09-15 &               0 (0) &          0.4 (0.0) \\
   276 &        H &       en &          2 &    560 | 1,118 &      EUR &  2018-09-15|2018-09-15 &               0 (0) &         0.45 (0.0) \\
   277 &        A &       en &          2 &      635 | 674 &      USD &  2019-01-25|2019-01-25 &               0 (0) &         0.99 (0.0) \\
   293 &        E &       fr &          2 &      250 | 577 &      USD &  2018-09-14|2018-11-09 &               0 (0) &         0.48 (0.0) \\
   298 &        A &       cs &          2 &      284 | 285 &      EUR &  2018-12-15|2018-12-15 &               0 (0) &         0.97 (0.0) \\
   388 &        F &       sv &          1 &      728 | 728 &      EUR &  2019-01-22|2019-01-22 &               0 (0) &          0.0 (0.0) \\
   416 &        M &       en &          1 &      815 | 815 &      USD &  2019-01-16|2019-01-16 &               0 (0) &          0.0 (0.0) \\
   485 &        M &       en &          1 &  1,000 | 1,000 &      USD &  2018-09-20|2018-09-20 &               0 (0) &          0.0 (0.0) \\
   518 &        H &       en &          1 &      448 | 448 &      EUR &  2018-09-15|2018-09-15 &               0 (0) &          0.0 (0.0) \\
   531 &       GG &       en &          1 &      700 | 700 &      USD &  2018-11-25|2018-11-25 &               0 (0) &          0.0 (0.0) \\
   717 &        B &       en &          1 &  3,000 | 3,000 &      USD &  2018-10-28|2018-10-28 &               0 (0) &          0.0 (0.0) \\
  1084 &        C &       ja &          1 &      562 | 562 &      USD &  2018-12-04|2018-12-04 &               0 (0) &          0.0 (0.0) \\
  1376 &        A &       en &          1 &      750 | 750 &      USD &  2019-01-15|2019-01-15 &               0 (0) &          0.0 (0.0) \\
  1378 &        H &       en &          1 &      560 | 560 &      EUR &  2018-09-15|2018-09-15 &               0 (0) &          0.0 (0.0) \\
  1420 &        A &       cs &          1 &      286 | 286 &      EUR &  2018-12-15|2018-12-15 &               0 (0) &          0.0 (0.0) \\
  1619 &        Q &       en &          1 &      895 | 895 &      USD &  2018-11-08|2018-11-08 &               0 (0) &          0.0 (0.0) \\
  1644 &        R &       en &          1 &      695 | 695 &      USD &  2019-01-18|2019-01-18 &               0 (0) &          0.0 (0.0) \\
  1748 &        R &       en &          1 &  1,000 | 1,000 &      USD &  2018-12-28|2018-12-28 &               0 (0) &          0.0 (0.0) \\
  1799 &        A &       cs &          1 &      286 | 286 &      EUR &  2018-12-16|2018-12-16 &               0 (0) &          0.0 (0.0) \\
\bottomrule
\end{tabular}


==> tables/short_basket_seeds_clusters_expanded.tex <==
\begin{tabular}{rrrr}
\toprule
Basket & \#Seed Addresses & \#Clusters & \#Expanded Addresses \\
\midrule
     0 &               2 &         2 &                  23 \\
     1 &               4 &         3 &                  85 \\
     2 &              46 &        44 &             398,816 \\
     3 &              17 &         9 &                  52 \\
     4 &              21 &        19 &                  27 \\
     5 &               1 &         1 &                  28 \\
     6 &               1 &         1 &                  36 \\
     7 &               2 &         2 &                  34 \\
     8 &              30 &        23 &                   0 \\
     9 &               8 &         4 &                  33 \\
    10 &               2 &         2 &                  25 \\
    11 &               4 &         3 &                  62 \\
    12 &              22 &        21 &                  68 \\
    13 &               3 &         3 &                  24 \\
    14 &          10,460 &    10,459 &                   0 \\
\bottomrule
\end{tabular}

